Robust Economic Model Predictive Control without Terminal Conditions

In this paper, a novel tube-based economic Model Predictive Control (MPC) scheme for uncertain systems that uses neither terminal costs nor terminal constraints is investigated. We show that the results from the undisturbed case can be extended to systems with bounded disturbances by using similar turnpike arguments and a properly modified stage cost. We prove robust guarantees on the closed-loop performance, convergence, and stability under suitable dissipativity and controllability conditions and discuss them in a numerical example.

==> sections/contour_plot_data.tex <==
\addplot[contour prepared, contour prepared format=matlab, line width=1.0pt, contour/draw color=black,contour/label distance={5.55cm}, contour/contour label style={every node/.append style={text=black}}, forget plot] table[row sep=crcr] {%
	-1.8	215\\
	3.36002999177146	1.5\\
	3.38	1.51522024396703\\
	3.38629093991859	1.52\\
	3.4	1.53040765063654\\
	3.4126741442043	1.54\\
	3.42	1.54554006728685\\
	3.43917935209422	1.56\\
	3.44	1.56061820862966\\
	3.46	1.57562834148247\\
	3.46584296676348	1.58\\
	3.48	1.59058335262543\\
	3.49263364434784	1.6\\
	3.5	1.6054859794207\\
	3.51954590699317	1.62\\
	3.52	1.62033690403182\\
	3.54	1.63512068326147\\
	3.54662020539548	1.64\\
	3.56	1.64985278783463\\
	3.57381870639974	1.66\\
	3.58	1.66453499292203\\
	3.6	1.67916519478852\\
	3.60114523861744	1.68\\
	3.62	1.6937315944567\\
	3.62863076850724	1.7\\
	3.64	1.70824983627741\\
	3.65623712598658	1.72\\
	3.66	1.72272055120049\\
	3.68	1.73713490226282\\
	3.68398772666791	1.74\\
	3.7	1.75149377426774\\
	3.71188147084186	1.76\\
	3.72	1.76580678317754\\
	3.7398954232681	1.78\\
	3.74	1.78007453328253\\
	3.76	1.79427872118723\\
	3.76807643371516	1.8\\
	3.78	1.80843840901044\\
	3.79637791985129	1.82\\
	3.8	1.82255442928821\\
	3.82	1.83661618685955\\
	3.82482673692073	1.84\\
	3.84	1.85062679438598\\
	3.85341610221631	1.86\\
	3.86	1.86459527525262\\
	3.88	1.87851729667158\\
	3.88213674168366	1.88\\
	3.9	1.8923829276205\\
	3.91101422305045	1.9\\
	3.92	1.90620792487799\\
	3.94	1.91999281034266\\
	3.94001046618417	1.92\\
	3.96	1.93371743798847\\
	3.96917619743895	1.94\\
	3.98	1.94740287929906\\
	3.99846017334253	1.96\\
	4	1.96104966421269\\
	4.02	1.97464061291716\\
	4.02790561938254	1.98\\
	4.04	1.98819030388185\\
	4.05747739313723	2\\
	4.06	2.00170272741452\\
	4.08	2.01516241413241\\
	4.0872057772637	2.02\\
	4.1	2.02858004400327\\
	4.1170652634098	2.04\\
	4.12	2.04196175469702\\
	4.14	2.05529249283355\\
	4.14707966834157	2.06\\
	4.16	2.06858163988668\\
	4.17722669393194	2.08\\
	4.18	2.08183617718172\\
	4.2	2.09504020396836\\
	4.20753001234822	2.1\\
	4.22	2.10820434056201\\
	4.23796432103085	2.12\\
	4.24	2.12133513974636\\
	4.26	2.13441461967309\\
	4.26855926425246	2.14\\
	4.28	2.14745711701355\\
	4.29928052009841	2.16\\
	4.3	2.16046751388799\\
	4.32	2.173424541937\\
	4.33016962625195	2.18\\
	4.34	2.18634867457281\\
	4.36	2.19923939915219\\
	4.36118350193005	2.2\\
	4.38	2.21207851454588\\
	4.39236305904878	2.22\\
	4.4	2.22488746460926\\
	4.42	2.23765895841759\\
	4.42367557951957	2.24\\
	4.44	2.2503848343546\\
	4.45514129245954	2.26\\
	4.46	2.26308169556748\\
	4.48	2.27573588626452\\
	4.4867545666872	2.28\\
	4.5	2.28835156193461\\
	4.51850583540611	2.3\\
	4.52	2.30093934339526\\
	4.54	2.31347809936773\\
	4.55042182536798	2.32\\
	4.56	2.32598653163865\\
	4.58	2.33846308749576\\
	4.58247016096078	2.34\\
	4.6	2.35089329424555\\
	4.61467851220415	2.36\\
	4.62	2.36329736112162\\
	4.64	2.37566135954458\\
	4.64703312645495	2.38\\
	4.66	2.38798895645589\\
	4.67952558707812	2.4\\
	4.68	2.40029146035334\\
	4.7	2.4125446265539\\
	4.71218807610499	2.42\\
	4.72	2.42477236930533\\
	4.74	2.43696602141588\\
	4.74498769650074	2.44\\
	4.76	2.44912004842628\\
	4.77793565528436	2.46\\
	4.78	2.46125062210298\\
	4.8	2.47333610172943\\
	4.81104612813455	2.48\\
	4.82	2.48539459604731\\
	4.84	2.49742210596044\\
	4.84429653564061	2.5\\
	4.86	2.50940952185792\\
	4.87769892736495	2.52\\
	4.88	2.52137505885785\\
	4.9	2.53329693322488\\
	4.91126282861113	2.54\\
	4.92	2.54519296038166\\
	4.94	2.55705833829708\\
	4.94496924272376	2.56\\
	4.96	2.56888581488693\\
	4.97882475678043	2.58\\
	4.98	2.58069292596827\\
	5	2.59245509016179\\
	5.01284699127117	2.6\\
	5.02	2.60419515570714\\
	5.04	2.61590223004129\\
	5.04701410607467	2.62\\
	5.06	2.62757617024542\\
	5.08	2.63922865497589\\
	5.08132718926158	2.64\\
	5.1	2.65083737553869\\
	5.11580616933582	2.66\\
	5.12	2.66242772650428\\
	5.14	2.67398015505268\\
	5.15043818653647	2.68\\
	5.16	2.68550670957591\\
	5.18	2.69700587028752\\
	5.18521826458453	2.7\\
	5.2	2.70846949823475\\
	5.22	2.71991586128635\\
	5.22014738391372	2.72\\
	5.24	2.7313174192156\\
	5.25524739357039	2.74\\
	5.26	2.74270250191681\\
	5.28	2.75405177859773\\
	5.29049802518047	2.76\\
	5.3	2.76537613940522\\
	5.32	2.77667386227486\\
	5.32589953867079	2.78\\
	5.34	2.78793832482249\\
	5.36	2.79918493641152\\
	5.36145281572707	2.8\\
	5.38	2.8103903120892\\
	5.39717087548922	2.82\\
	5.4	2.82158101379829\\
	5.42	2.83273333611657\\
	5.43304775229352	2.84\\
	5.44	2.84386623006631\\
	5.46	2.85496861322892\\
	5.46907800199832	2.86\\
	5.48	2.86604448049838\\
	5.5	2.87709734157423\\
	5.50526241548086	2.88\\
	5.52	2.88811695195595\\
	5.54	2.899120701523\\
	5.54160175860107	2.9\\
	5.56	2.91008481377228\\
	5.57810469716143	2.92\\
	5.58	2.92103642456981\\
	5.6	2.93194921813322\\
	5.61476990702529	2.94\\
	5.62	2.94284652942681\\
	5.64	2.95371130044736\\
	5.65159138432325	2.96\\
	5.66	2.96455504364929\\
	5.68	2.97537217970608\\
	5.68856981313848	2.98\\
	5.7	2.98616307603069\\
	5.72	2.99693295883364\\
	5.72570585497768	3\\
	5.74	3.00767171951632\\
	5.76	3.01839472502781\\
	5.76300014927538	3.02\\
	5.78	3.02908205153803\\
	5.8	3.03975855009127\\
	5.80045331388342	3.04\\
	5.82	3.05039513433978\\
	5.83807369238283	3.06\\
	5.84	3.06102210666483\\
	5.86	3.0716120152946\\
	5.8758551909358	3.08\\
	5.88	3.08218934170647\\
	5.9	3.09273372721307\\
	5.91379655015043	3.1\\
	5.92	3.10326207592353\\
	5.94	3.11376128864361\\
	5.95189831718073	3.12\\
	5.96	3.1242413190053\\
	5.98	3.13469570416493\\
	5.99016101960832	3.14\\
	6.1	3.19512806685441\\
};

\addplot[contour prepared, contour prepared format=matlab, line width=1.0pt, contour/draw color=black,contour/label distance={6.3cm}, contour/contour label style={every node/.append style={text=black}}, forget plot] table[row sep=crcr] {%
	-1.6	333\\
	2.11770967882539	1.5\\
	2.12	1.502378781572\\
	2.13707434097858	1.52\\
	2.14	1.52301975745262\\
	2.15655484863239	1.54\\
	2.16	1.54353404601649\\
	2.17615164694768	1.56\\
	2.18	1.56392355036343\\
	2.19586515739813	1.58\\
	2.2	1.58419013651553\\
	2.21569577847053	1.6\\
	2.22	1.60433563448696\\
	2.23564388633798	1.62\\
	2.24	1.62436183931426\\
	2.25570983550713	1.64\\
	2.26	1.64427051204897\\
	2.27589395944068	1.66\\
	2.28	1.6640633807142\\
	2.29619657115623	1.68\\
	2.3	1.68374214122683\\
	2.31661796380276	1.7\\
	2.32	1.70330845828671\\
	2.33715841121536	1.72\\
	2.34	1.72276396623452\\
	2.35781816844958	1.74\\
	2.36	1.74211026987939\\
	2.37859747229606	1.76\\
	2.38	1.76134894529784\\
	2.39949654177633	1.78\\
	2.4	1.78048154060504\\
	2.42	1.79950759219562\\
	2.42052038853213	1.8\\
	2.44	1.81842821198108\\
	2.44167009735168	1.82\\
	2.46	1.83724682213901\\
	2.46294108827859	1.84\\
	2.48	1.85596487139821\\
	2.48433349611851	1.86\\
	2.5	1.87458378386933\\
	2.50584744058969	1.88\\
	2.52	1.89310495967755\\
	2.52748302670686	1.9\\
	2.54	1.91152977557466\\
	2.5492403451518	1.92\\
	2.56	1.92985958553121\\
	2.57111947263114	1.94\\
	2.58	1.94809572130962\\
	2.59312047222202	1.96\\
	2.6	1.96623949301897\\
	2.61524339370595	1.98\\
	2.62	1.98429218965215\\
	2.63748827389146	2\\
	2.64	2.00225507960612\\
	2.65985513692584	2.02\\
	2.66	2.02012941118589\\
	2.68	2.03790797910734\\
	2.68236402309617	2.04\\
	2.7	2.05559954621418\\
	2.70499692214664	2.06\\
	2.72	2.07320583084046\\
	2.72775256334315	2.08\\
	2.74	2.09072800939987\\
	2.75063091031603	2.1\\
	2.76	2.10816724041825\\
	2.77363191574742	2.12\\
	2.78	2.12552466495468\\
	2.79675552161743	2.14\\
	2.8	2.14280140701026\\
	2.82	2.15999856815457\\
	2.82000167301199	2.16\\
	2.84	2.17710558604173\\
	2.8433976496153	2.18\\
	2.86	2.19413486741285\\
	2.86691666477711	2.2\\
	2.88	2.21108747502075\\
	2.89055860915166	2.22\\
	2.9	2.22796445635498\\
	2.91432336405464	2.24\\
	2.92	2.24476684398629\\
	2.93821080165923	2.26\\
	2.94	2.26149565590133\\
	2.96	2.2781444153916\\
	2.96223820807189	2.28\\
	2.98	2.29471523430693\\
	2.98640273995326	2.3\\
	3	2.31121514124871\\
	3.01069011907537	2.32\\
	3.02	2.32764510166257\\
	3.03510017365802	2.34\\
	3.04	2.34400606788556\\
	3.05963272387273	2.36\\
	3.06	2.36029897943047\\
	3.08	2.37651069215498\\
	3.08432009830721	2.38\\
	3.1	2.39265469008258\\
	3.10913293996972	2.4\\
	3.12	2.40873308784017\\
	3.13406823754558	2.42\\
	3.14	2.42474677860755\\
	3.15912577246118	2.44\\
	3.16	2.44069664399763\\
	3.18	2.45656972139975\\
	3.18433708913399	2.46\\
	3.2	2.47237760475685\\
	3.20967718165049	2.48\\
	3.22	2.48812396277175\\
	3.23513931929944	2.5\\
	3.24	2.50380963516616\\
	3.26	2.51943316671306\\
	3.26072847205579	2.52\\
	3.28	2.53498198784471\\
	3.28647491596236	2.54\\
	3.3	2.55047231171657\\
	3.3123431006443	2.56\\
	3.32	2.56590493929258\\
	3.3383327467118	2.58\\
	3.34	2.5812806618587\\
	3.36	2.5965864960096\\
	3.36447485241959	2.6\\
	3.38	2.61183153836731\\
	3.39075008374439	2.62\\
	3.4	2.62702173433556\\
	3.41714634453916	2.64\\
	3.42	2.64215783999681\\
	3.44	2.65722943156722\\
	3.44368860252082	2.66\\
	3.46	2.6722394384832\\
	3.47037146862469	2.68\\
	3.48	2.68719731950689\\
	3.49717483793772	2.7\\
	3.5	2.70210379803908\\
	3.52	2.71694727989676\\
	3.52412611015604	2.72\\
	3.54	2.73173202674689\\
	3.55121681762007	2.74\\
	3.56	2.7464672479075\\
	3.57842741436859	2.76\\
	3.58	2.76115363639719\\
	3.6	2.7757748365835\\
	3.6057957715703	2.78\\
	3.62	2.79034366073186\\
	3.6332941724223	2.8\\
	3.64	2.80486544741657\\
	3.66	2.81933819407088\\
	3.66091773341584	2.82\\
	3.68	2.83374532340152\\
	3.68870454392702	2.84\\
	3.7	2.84810715404989\\
	3.71661016005663	2.86\\
	3.72	2.8624243310882\\
	3.74	2.8766841216328\\
	3.74466397803829	2.88\\
	3.76	2.89089049431858\\
	3.7728580437435	2.9\\
	3.78	2.9050538798182\\
	3.8	2.91917155914346\\
	3.80117750545356	2.92\\
	3.82	2.93322683131211\\
	3.82966032166057	2.94\\
	3.84	2.94724073255999\\
	3.85826063630556	2.96\\
	3.86	2.96121386544706\\
	3.88	2.97512717078284\\
	3.88702150624129	2.98\\
	3.9	2.98899576346126\\
	3.91591023355392	3\\
	3.92	3.0028251396433\\
	3.94	3.01660217770107\\
	3.94494573789783	3.02\\
	3.96	3.03032951199441\\
	3.97412290807864	3.04\\
	3.98	3.04401913691008\\
	4	3.05766219184446\\
	4.00343680293874	3.06\\
	4.02	3.07125219819029\\
	4.03290233849238	3.08\\
	4.04	3.08480595959614\\
	4.06	3.09831724248972\\
	4.06249815034532	3.1\\
	4.08	3.11177373699953\\
	4.0922518711299	3.12\\
	4.1	3.12519541027246\\
	4.12	3.13857706226918\\
	4.12213290749315	3.14\\
	4.14	3.15190375184157\\
	4.15217453544584	3.16\\
	4.16	3.16519700498219\\
	4.18	3.17845110024956\\
	4.1823438948974	3.18\\
	4.2	3.19165158739724\\
	4.21267305846029	3.2\\
	4.22	3.20481998575449\\
	4.24	3.21794853428571\\
	4.2431336400537	3.22\\
	4.26	3.23102632169577\\
	4.27374987832197	3.24\\
	4.28	3.24407333243186\\
	4.3	3.25707828269819\\
	4.30450439044007	3.26\\
	4.32	3.27003677754356\\
	4.33540715705261	3.28\\
	4.34	3.28296577385643\\
	4.36	3.2958490153194\\
	4.36645812574	3.3\\
	4.38	3.30869153333802\\
	4.39764679253082	3.32\\
	4.4	3.32150579845751\\
	4.42	3.33426916394972\\
	4.42899656934162	3.34\\
	4.44	3.34699893330672\\
	4.46	3.35970045710692\\
	4.4604730331027	3.36\\
	4.48	3.37234693226196\\
	4.49212119916323	3.38\\
	4.5	3.38496709720892\\
	4.52	3.3975515367924\\
	4.52390070370111	3.4\\
	4.54	3.4100903051894\\
	4.55583325785168	3.42\\
	4.56	3.42260392953375\\
	4.58	3.43507298174076\\
	4.5879177212511	3.44\\
	4.6	3.44750705783036\\
	4.62	3.45991679291289\\
	4.62013448091596	3.46\\
	4.64	3.47227244084132\\
	4.65252495352851	3.48\\
	4.66	3.48460476389927\\
	4.68	3.49690169964173\\
	4.68505021311674	3.5\\
	4.7	3.5091573665999\\
	4.71772305770277	3.52\\
	4.72	3.52139080375279\\
	4.74	3.53357651417797\\
	4.75055834768587	3.54\\
	4.76	3.5457350229159\\
	4.78	3.55786375968375\\
	4.78353082601386	3.56\\
	4.8	3.56994838675093\\
	4.81665920557222	3.58\\
	4.82	3.58201249247548\\
	4.84	3.59403240769279\\
	4.84994463556906	3.6\\
	4.86	3.60602429075871\\
	4.88	3.61798857485159\\
	4.88337011987656	3.62\\
	4.9	3.62990924022316\\
	4.91695248229041	3.64\\
	4.92	3.64181102958857\\
	4.94	3.65366879177758\\
	4.95069348258875	3.66\\
	4.96	3.66550095799488\\
	4.98	3.67730437437115\\
	4.98457716531284	3.68\\
	5	3.68906788313275\\
	5.01861169254976	3.7\\
	5.02	3.70081410206571\\
	5.04	3.71251319798515\\
	5.0528131209854	3.72\\
	5.06	3.72419229343055\\
	5.08	3.73583827484133\\
	5.0871596368442	3.74\\
	5.1	3.74745117554011\\
	5.12	3.7590444657383\\
	5.12165236203707	3.76\\
	5.14	3.77059208678953\\
	5.15631043827913	3.78\\
	5.16	3.78212451058627\\
	5.18	3.7936163460553\\
	5.19112389827248	3.8\\
	5.2	3.80508494603264\\
	5.22	3.81652525310561\\
	5.22608568111197	3.82\\
	5.24	3.8279309103402\\
	5.26	3.8393200890001\\
	5.26119679477956	3.84\\
	5.28	3.85066367198802\\
	5.29647508095156	3.86\\
	5.3	3.86199405158608\\
	5.32	3.87328448141034\\
	5.3319093475695	3.88\\
	5.34	3.88455417065574\\
	5.36	3.89579457136873\\
	5.36749479089463	3.9\\
	5.38	3.90700440737761\\
	5.4	3.91819515731467\\
	5.40323231416232	3.92\\
	5.42	3.92934596558162\\
	5.43912687946505	3.94\\
	5.44	3.94048547365641\\
	5.46	3.9515800323894\\
	5.47518944884796	3.96\\
	5.48	3.96266183028484\\
	5.5	3.97370777855231\\
	5.51140569769638	3.98\\
	5.52	3.98473266277269\\
	5.54	3.99573035878104\\
	5.54777643270966	4\\
	5.56	4.00669911507765\\
	5.58	4.01764891206705\\
	5.58430243400752	4.02\\
	5.6	4.0285623156634\\
	5.62	4.03946456199609\\
	5.62098445572878	4.04\\
	5.64	4.05032337780726\\
	5.65783303942116	4.06\\
	5.66	4.06117366938762\\
	5.68	4.07198339990027\\
	5.69484266394638	4.08\\
	5.7	4.08278032774724\\
	5.72	4.09354346574005\\
	5.73200955728948	4.1\\
	5.74	4.1042877690559\\
	5.76	4.11500464481644\\
	5.7693343883357	4.12\\
	5.78	4.12569705324308\\
	5.8	4.13636799259038\\
	5.8068178024441	4.14\\
	5.82	4.1470092264038\\
	5.84	4.15763455076593\\
	5.84446042195562	4.16\\
	5.86	4.16822532106578\\
	5.88	4.17880534755593\\
	5.88226284668648	4.18\\
	5.9	4.18934635645031\\
	5.92	4.1998813979412\\
	5.92022565440736	4.2\\
	5.94	4.21037333872687\\
	5.95835652906522	4.22\\
	5.96	4.22086022396935\\
	5.98	4.23130726126175\\
	5.99664907318776	4.24\\
	6	4.24174619198764\\
};

\addplot[contour prepared, contour prepared format=matlab, line width=1.0pt, contour/draw color=black,contour/label distance={7.2cm}, contour/contour label style={every node/.append style={text=black}}, forget plot] table[row sep=crcr] {%
	-1.4	325\\
	1.36303125044718	1.5\\
	1.37751142784742	1.52\\
	1.38	1.5234401516118\\
	1.39211676892836	1.54\\
	1.4	1.55079350307881\\
	1.40679994543824	1.56\\
	1.42	1.5779029447301\\
	1.4215633065625	1.58\\
	1.43646522061827	1.6\\
	1.44	1.60474964911805\\
	1.4514731692113	1.62\\
	1.46	1.63135251015342\\
	1.46656457976557	1.64\\
	1.48	1.65772619220537\\
	1.48174153098528	1.66\\
	1.49705121148748	1.68\\
	1.5	1.68385587377952\\
	1.51247391599205	1.7\\
	1.52	1.70975469118252\\
	1.5279849564887	1.72\\
	1.54	1.73543781049772\\
	1.54358617412598	1.74\\
	1.5592898601445	1.76\\
	1.56	1.76090462978381\\
	1.57513737712269	1.78\\
	1.58	1.78614201310829\\
	1.59107744278198	1.8\\
	1.6	1.8111760787856\\
	1.60711168854416	1.82\\
	1.62	1.83601038340334\\
	1.62324167917963	1.84\\
	1.63947634971592	1.86\\
	1.64	1.86064520597363\\
	1.65585307252748	1.88\\
	1.66	1.88506847062894\\
	1.6723274177992	1.9\\
	1.68	1.90930310382508\\
	1.68890077152264	1.92\\
	1.7	1.93335230628995\\
	1.70557446256391	1.94\\
	1.72	1.95721920318449\\
	1.72234976479843	1.96\\
	1.73923817818512	1.98\\
	1.74	1.9809023861418\\
	1.75625998709454	2\\
	1.76	2.00439650507067\\
	1.77338476402723	2.02\\
	1.78	2.02771814496375\\
	1.79061363491995	2.04\\
	1.8	2.05087013518676\\
	1.80794767814639	2.06\\
	1.82	2.07385524199665\\
	1.82538792619643	2.08\\
	1.84	2.09667617058675\\
	1.84293536727839	2.1\\
	1.86	2.11933556704778\\
	1.86059094684863	2.12\\
	1.87837607223666	2.14\\
	1.88	2.14182699141382\\
	1.89627667213663	2.16\\
	1.9	2.16415951951547\\
	1.91428617826057	2.18\\
	1.92	2.18633888570766\\
	1.93240542060977	2.2\\
	1.94	2.20836750339054\\
	1.95063519178566	2.22\\
	1.96	2.23024773601612\\
	1.96897624821351	2.24\\
	1.98	2.25198189860525\\
	1.9874293113137	2.26\\
	2	2.27357225920632\\
	2.00599506862327	2.28\\
	2.02	2.29502104029813\\
	2.02467417487029	2.3\\
	2.04	2.31633042013977\\
	2.04346725300341	2.32\\
	2.06	2.33750253406978\\
	2.06237489517885	2.34\\
	2.08	2.358539475757\\
	2.08139766370696	2.36\\
	2.1	2.37944329840517\\
	2.10053609196027	2.38\\
	2.11979304391428	2.4\\
	2.12	2.40021495320886\\
	2.13917129051528	2.42\\
	2.14	2.42085537578369\\
	2.15866522307045	2.44\\
	2.16	2.44136923385083\\
	2.17827529627433	2.46\\
	2.18	2.46175842011906\\
	2.19800193907994	2.48\\
	2.2	2.48202479252596\\
	2.21784555544231	2.5\\
	2.22	2.50217017519465\\
	2.23780652503331	2.52\\
	2.24	2.52219635935713\\
	2.25788520392893	2.54\\
	2.26	2.54210510424589\\
	2.27808192527037	2.56\\
	2.28	2.56189813795497\\
	2.2983969999002	2.58\\
	2.3	2.5815771582717\\
	2.31883071697451	2.6\\
	2.32	2.6011438334805\\
	2.33938334455236	2.62\\
	2.34	2.62059980313976\\
	2.36	2.63994641520151\\
	2.36005570375921	2.64\\
	2.38	2.6591820197655\\
	2.38085504458014	2.66\\
	2.4	2.67831114680307\\
	2.40177509212114	2.68\\
	2.42	2.69733533514313\\
	2.42281601503073	2.7\\
	2.44	2.71625609821347\\
	2.44397796403825	2.72\\
	2.46	2.73507492468394\\
	2.4652610724078	2.74\\
	2.48	2.75379327908911\\
	2.48666545637606	2.76\\
	2.5	2.77241260243134\\
	2.50819121557481	2.78\\
	2.52	2.79093431276483\\
	2.52983843343867	2.8\\
	2.54	2.80935980576157\\
	2.55160717759868	2.82\\
	2.56	2.82769045525976\\
	2.57349750026234	2.84\\
	2.58	2.84592761379535\\
	2.59550943858057	2.86\\
	2.6	2.8640726131175\\
	2.6176430150022	2.88\\
	2.62	2.88212676468833\\
	2.63989823761642	2.9\\
	2.64	2.90009136016775\\
	2.66	2.91795761868113\\
	2.66229649689866	2.92\\
	2.68	2.9357359529294\\
	2.68481820619769	2.94\\
	2.7	2.95342805429759\\
	2.70746235524982	2.96\\
	2.72	2.97103514435626\\
	2.73022888394879	2.98\\
	2.74	2.98855842697094\\
	2.75311771971009	3\\
	2.76	3.00599908871107\\
	2.77612877774063	3.02\\
	2.78	3.02335829924724\\
	2.79926196129948	3.04\\
	2.8	3.04063721173719\\
	2.82	3.05782626308195\\
	2.82253969741181	3.06\\
	2.84	3.07493371861103\\
	2.84594673420258	3.08\\
	2.86	3.09196383789125\\
	2.86947628377387	3.1\\
	2.88	3.10891771534282\\
	2.89312819251734	3.12\\
	2.9	3.12579643055095\\
	2.91690229632371	3.14\\
	2.92	3.14260104859425\\
	2.94	3.15932932019236\\
	2.9408053212379	3.16\\
	2.96	3.17597234791092\\
	2.96485778739663	3.18\\
	2.98	3.19254401009136\\
	2.98903257414616	3.2\\
	3	3.20904532001573\\
	3.01332946735756	3.22\\
	3.02	3.22547727789224\\
	3.03774824359591	3.24\\
	3.04	3.2418408711363\\
	3.06	3.25812785980403\\
	3.06230779918375	3.26\\
	3.08	3.27433896095674\\
	3.08700830804397	3.28\\
	3.1	3.29048422536796\\
	3.11183059495234	3.3\\
	3.12	3.30656459460401\\
	3.13677439215082	3.32\\
	3.14	3.32258099866874\\
	3.16	3.33852710724733\\
	3.16185438755851	3.34\\
	3.18	3.3543979759779\\
	3.18708228428689	3.36\\
	3.2	3.37020725667829\\
	3.21243141391922	3.38\\
	3.22	3.38595583777906\\
	3.23790146843062	3.4\\
	3.24	3.40164459723763\\
	3.26	3.41726091787579\\
	3.26351981314987	3.42\\
	3.28	3.43281067919509\\
	3.28927569807257	3.44\\
	3.3	3.44830285890125\\
	3.3151520740042	3.46\\
	3.32	3.46373829717304\\
	3.34	3.47911346212174\\
	3.34115751574478	3.48\\
	3.36	3.49441474657413\\
	3.36732108025159	3.5\\
	3.38	3.50966143022526\\
	3.39360458641314	3.52\\
	3.4	3.52485431816566\\
	3.42	3.53999417802554\\
	3.42000772061524	3.54\\
	3.44	3.55505753776106\\
	3.44657942682382	3.56\\
	3.46	3.57006914985013\\
	3.47327041796322	3.58\\
	3.48	3.5850297867556\\
	3.5	3.5999399171513\\
	3.50008089628586	3.6\\
	3.52	3.61477544717681\\
	3.52706077688604	3.62\\
	3.54	3.62956196376984\\
	3.55415918561333	3.64\\
	3.56	3.6443002090199\\
	3.58	3.65898592710132\\
	3.58138578272438	3.66\\
	3.6	3.6736032957526\\
	3.60877347050742	3.68\\
	3.62	3.68817427424041\\
	3.63627883609352	3.7\\
	3.64	3.70269957635007\\
	3.66	3.71716595607479\\
	3.66392951023892	3.72\\
	3.68	3.73157443301129\\
	3.69172426477053	3.74\\
	3.7	3.74593903945566\\
	3.71963575917133	3.76\\
	3.72	3.76026046279144\\
	3.74	3.77451234908793\\
	3.74771770720972	3.78\\
	3.76	3.78872083105142\\
	3.77591843896196	3.8\\
	3.78	3.80288786535874\\
	3.8	3.81699934113882\\
	3.80426442603806	3.82\\
	3.82	3.83105613664681\\
	3.83275459787242	3.84\\
	3.84	3.84507317119847\\
	3.86	3.85904639767148\\
	3.86136924917703	3.86\\
	3.88	3.87295581751612\\
	3.89014893041488	3.88\\
	3.9	3.886827116579\\
	3.91904309121466	3.9\\
	3.92	3.90066092400619\\
	3.94	3.91443042452485\\
	3.94810572370529	3.92\\
	3.96	3.92816013284248\\
	3.97728865564049	3.94\\
	3.98	3.94185392965611\\
	4	3.95549021124394\\
	4.00662887667686	3.96\\
	4.02	3.96908235922707\\
	4.03610036284538	3.98\\
	4.04	3.98264013413176\\
	4.06	3.99614514639392\\
	4.06572191806944	4\\
	4.08	4.00960365503752\\
	4.09548162750977	4.02\\
	4.1	4.02302928916624\\
	4.12	4.03640492565859\\
	4.12538802328651	4.04\\
	4.14	4.04973361120236\\
	4.15543551602426	4.06\\
	4.16	4.06303088267946\\
	4.18	4.07627898290524\\
	4.18563003020373	4.08\\
	4.2	4.08948156125357\\
	4.21596476197574	4.1\\
	4.22	4.10265414952354\\
	4.24	4.11577650084624\\
	4.24645045400563	4.12\\
	4.26	4.12885659176245\\
	4.27707178068503	4.14\\
	4.28	4.14190808169866\\
	4.3	4.15490642117433\\
	4.30785150112036	4.16\\
	4.32	4.167867552263\\
	4.33875868286404	4.18\\
	4.34	4.18080143806997\\
	4.36	4.19367745420243\\
	4.36983508231649	4.2\\
	4.38	4.20652306469265\\
	4.4	4.21933950355916\\
	4.40103362889736	4.22\\
	4.42	4.23209808803617\\
	4.43240282502058	4.24\\
	4.44	4.24483153237773\\
	4.46	4.25752817991244\\
	4.46390281795636	4.26\\
	4.48	4.27017659730621\\
	4.49555608490933	4.28\\
	4.5	4.28280114858986\\
	4.52	4.29537957759025\\
	4.52735967847257	4.3\\
	4.54	4.3079210514852\\
	4.55929595682566	4.32\\
	4.56	4.32043990469745\\
	4.58	4.33290164501701\\
	4.59140513412429	4.34\\
	4.6	4.34533932281304\\
	4.62	4.35774449509415\\
	4.62364477088059	4.36\\
	4.64	4.37010213793132\\
	4.65603986483923	4.38\\
	4.66	4.38243909385233\\
	4.68	4.39472987712314\\
	4.68858878895656	4.4\\
	4.7	4.40698862673391\\
	4.72	4.41922404641013\\
	4.72127168050834	4.42\\
	4.74	4.43140568618984\\
	4.75412408398638	4.44\\
	4.76	4.44356850349764\\
	4.78	4.45569174150698\\
	4.78711953046871	4.46\\
	4.8	4.46777920868852\\
	4.82	4.47984824200742\\
	4.82025216322034	4.48\\
	4.84	4.49186141410801\\
	4.85356004014368	4.5\\
};

\addplot[contour prepared, contour prepared format=matlab, line width=1.0pt, contour/draw color=black,contour/label distance={6.2cm}, contour/contour label style={every node/.append style={text=black}}, forget plot] table[row sep=crcr] {%
	-1.2		280\\
	1	1.66256677955626\\
	1.01034351527305	1.68\\
	1.02	1.69634262214706\\
	1.02219810988077	1.7\\
	1.03420527268462	1.72\\
	1.04	1.72968028863779\\
	1.04628107909401	1.74\\
	1.05841662299817	1.76\\
	1.06	1.76261156760387\\
	1.07071546705971	1.78\\
	1.08	1.79512302227253\\
	1.08304215491865	1.8\\
	1.095499694622	1.82\\
	1.1	1.82724082661627\\
	1.10805456385049	1.84\\
	1.12	1.85898927933991\\
	1.12064556917998	1.86\\
	1.13341628018332	1.88\\
	1.14	1.89034276486541\\
	1.14623981884216	1.9\\
	1.15912519666621	1.92\\
	1.16	1.92135839184677\\
	1.17218215134711	1.94\\
	1.18	1.95200146800326\\
	1.18528548866623	1.96\\
	1.19847015109796	1.98\\
	1.2	1.98232229196601\\
	1.21181024096086	2\\
	1.22	2.01229527331646\\
	1.22520315093241	2.02\\
	1.23867854015016	2.04\\
	1.24	2.041962468626\\
	1.25231094048279	2.06\\
	1.26	2.07129734212236\\
	1.26600198005675	2.08\\
	1.27975962780225	2.1\\
	1.28	2.10034947753097\\
	1.29369235682417	2.12\\
	1.3	2.12907616139938\\
	1.30768898595296	2.14\\
	1.32	2.15753470868101\\
	1.32175261094821	2.16\\
	1.33596053507043	2.18\\
	1.34	2.18569598510284\\
	1.35026922141453	2.2\\
	1.36	2.21358610526168\\
	1.36464941333573	2.22\\
	1.37911965235514	2.24\\
	1.38	2.24121722384568\\
	1.39374596295777	2.26\\
	1.4	2.26856454101155\\
	1.40844785103346	2.28\\
	1.42	2.29567089132346\\
	1.42322783414354	2.3\\
	1.43812086905376	2.32\\
	1.44	2.32252543444235\\
	1.45314880065499	2.34\\
	1.46	2.34912320767111\\
	1.46825830416838	2.36\\
	1.48	2.37549418316692\\
	1.4834516060876	2.38\\
	1.49875172628881	2.4\\
	1.5	2.40163252746495\\
	1.51419403271315	2.42\\
	1.52	2.42752640599439\\
	1.52972309310588	2.44\\
	1.54	2.45320652515078\\
	1.54534087791994	2.46\\
	1.56	2.47867654598704\\
	1.56104927666724	2.48\\
	1.57689972386264	2.5\\
	1.58	2.50391653120565\\
	1.59285811028612	2.52\\
	1.6	2.52894688194401\\
	1.60890946139035	2.54\\
	1.62	2.55377889096661\\
	1.62505544934732	2.56\\
	1.64	2.57841586470419\\
	1.64129767724391	2.58\\
	1.65767340458412	2.6\\
	1.66	2.60284395659189\\
	1.67416556335862	2.62\\
	1.68	2.62707513085762\\
	1.69075579769266	2.64\\
	1.7	2.65112192230573\\
	1.70744552461061	2.66\\
	1.72	2.67498733057512\\
	1.7242361017029	2.68\\
	1.74	2.69867429145506\\
	1.74112882929466	2.7\\
	1.75815196497914	2.72\\
	1.76	2.72217262836271\\
	1.77529376936318	2.74\\
	1.78	2.74549135411324\\
	1.79253901403473	2.76\\
	1.8	2.76864112546764\\
	1.80988884453258	2.78\\
	1.82	2.79162461950561\\
	1.82734435668326	2.8\\
	1.84	2.81444445918943\\
	1.84490659831306	2.82\\
	1.86	2.83710321493147\\
	1.86257657088257	2.84\\
	1.88	2.85960340610706\\
	1.88035523104813	2.86\\
	1.89826724225291	2.88\\
	1.9	2.88193587336945\\
	1.91629258074114	2.9\\
	1.92	2.90411323302561\\
	1.93442727502765	2.92\\
	1.94	2.92614021197313\\
	1.95267216005001	2.94\\
	1.96	2.94801912238304\\
	1.97102803140637	2.96\\
	1.98	2.96975223278302\\
	1.98949564660802	2.98\\
	2	2.99134176925981\\
	2.00807572627895	3\\
	2.02	3.01278991662142\\
	2.02676895530501	3.02\\
	2.04	3.03409881952061\\
	2.04557598393519	3.04\\
	2.06	3.05527058354124\\
	2.06449742883748	3.06\\
	2.08	3.07630727624883\\
	2.08353387411149	3.08\\
	2.1	3.09721092820666\\
	2.1026858722599	3.1\\
	2.12	3.11798353395886\\
	2.12195394512088	3.12\\
	2.14	3.13862705298154\\
	2.14133858476309	3.14\\
	2.16	3.15914341060332\\
	2.16084025434539	3.16\\
	2.18	3.17953449889635\\
	2.18045938894252	3.18\\
	2.2	3.19980217753891\\
	2.20019639633866	3.2\\
	2.22	3.2199482746507\\
	2.22005165779021	3.22\\
	2.24	3.2399745876018\\
	2.24002552875918	3.24\\
	2.26	3.25988288379632\\
	2.26011833961858	3.26\\
	2.28	3.27967490143158\\
	2.28033039633105	3.28\\
	2.3	3.29935235023385\\
	2.30066198110192	3.3\\
	2.32	3.31891691217145\\
	2.32111335300782	3.32\\
	2.34	3.33837024214597\\
	2.34168474860194	3.34\\
	2.36	3.35771396866254\\
	2.3623763824969	3.36\\
	2.38	3.37694969447981\\
	2.38318844792628	3.38\\
	2.4	3.39607899724042\\
	2.40412111728563	3.4\\
	2.42	3.41510343008261\\
	2.4251745426539	3.42\\
	2.44	3.43402452223373\\
	2.44634885629604	3.44\\
	2.46	3.4528437795862\\
	2.46764417114762	3.46\\
	2.48	3.47156268525659\\
	2.48906058128224	3.48\\
	2.5	3.49018270012847\\
	2.51059816236226	3.5\\
	2.52	3.50870526337942\\
	2.53225697207377	3.52\\
	2.54	3.52713179299303\\
	2.55403705054627	3.54\\
	2.56	3.5454636862561\\
	2.5759384207577	3.56\\
	2.58	3.56370232024186\\
	2.59796108892544	3.58\\
	2.6	3.5818490522794\\
	2.62	3.59990465070329\\
	2.62010614660764	3.6\\
	2.64	3.6178593457413\\
	2.64239497380517	3.62\\
	2.66	3.63572555188474\\
	2.66480599855208	3.64\\
	2.68	3.65350455758093\\
	2.68733914800402	3.66\\
	2.7	3.67119763353142\\
	2.70999433470317	3.68\\
	2.72	3.68880603309348\\
	2.73277145688429	3.7\\
	2.74	3.70633099267067\\
	2.75567039877044	3.72\\
	2.76	3.72377373209293\\
	2.77869103085891	3.74\\
	2.78	3.74113545498642\\
	2.8	3.75840783177252\\
	2.80185141285489	3.76\\
	2.82	3.775594228721\\
	2.8251471141356	3.78\\
	2.84	3.79270262997501\\
	2.84856488388949	3.8\\
	2.86	3.80973418220117\\
	2.87210452782338	3.82\\
	2.88	3.82669001744676\\
	2.89576583950675	3.84\\
	2.9	3.84357125345827\\
	2.9195486005972	3.86\\
	2.92	3.86037899399187\\
	2.94	3.87709696914334\\
	2.94348551653507	3.88\\
	2.96	3.89374086869217\\
	2.96754851060329	3.9\\
	2.98	3.9103140376046\\
	2.9917329909825	3.92\\
	3	3.92681753016242\\
	3.01603868315592	3.94\\
	3.02	3.94325238799285\\
	3.04	3.9596173538523\\
	3.040469618228	3.96\\
	3.06	3.97589575232717\\
	3.06505882656297	3.98\\
	3.08	3.99210812175183\\
	3.08976906734191	4\\
	3.1	4.00825545880139\\
	3.11460001503947	4.02\\
	3.12	4.02433874868674\\
	3.13955133437618	4.04\\
	3.14	4.04035896539432\\
	3.16	4.05629491037414\\
	3.16466423893909	4.06\\
	3.18	4.07216711118388\\
	3.18990152708968	4.08\\
	3.2	4.0879786695217\\
	3.21525877468761	4.1\\
	3.22	4.10373051928988\\
	3.24	4.11942011894727\\
	3.24074207601033	4.12\\
	3.26	4.13502903352783\\
	3.26638710928137	4.14\\
	3.28	4.15058056710714\\
	3.29215154809669	4.16\\
	3.3	4.16607561630431\\
	3.31803497760099	4.18\\
	3.32	4.18151506829082\\
	3.34	4.19688114921749\\
	3.34407164953463	4.2\\
	3.36	4.21218387454207\\
	3.37024399028382	4.22\\
	3.38	4.22743320862362\\
	3.396534604454	4.24\\
	3.4	4.24263000460726\\
	3.42	4.25776172493301\\
	3.42296782686231	4.26\\
	3.44	4.27282639955843\\
	3.44954826708888	4.28\\
	3.46	4.28784065368403\\
	3.47624614252611	4.3\\
	3.48	4.30280530875002\\
	3.5	4.31770747151322\\
	3.50308626833648	4.32\\
	3.52	4.33254442308367\\
	3.53007452753647	4.34\\
	3.54	4.34733381049772\\
	3.55717927055722	4.36\\
	3.56	4.36207642563345\\
	3.58	4.37675363788974\\
	3.5844356906904	4.38\\
	3.6	4.39137279106128\\
	3.61183104194776	4.4\\
	3.62	4.40594712941735\\
	3.63934181942557	4.42\\
	3.64	4.42047741725448\\
	3.66	4.43493409858301\\
	3.6670230282954	4.44\\
	3.68	4.4493450000058\\
	3.69482432681793	4.46\\
	3.7	4.46371373580253\\
	3.72	4.47802926289343\\
	3.72276143613043	4.48\\
	3.74	4.49228143522784\\
	3.75085354902169	4.5\\
};

\addplot[contour prepared, contour prepared format=matlab, line width=1.0pt, contour/draw color=black,contour/label distance={4.3cm}, contour/contour label style={every node/.append style={text=black}}, forget plot] table[row sep=crcr] {%
	-1	209\\
	1	2.28171238786219\\
	1.01085553917348	2.3\\
	1.02	2.31548339352669\\
	1.02271573553556	2.32\\
	1.0347216162354	2.34\\
	1.04	2.34882177591587\\
	1.0468065944149	2.36\\
	1.05893513432265	2.38\\
	1.06	2.3817571390405\\
	1.07124679714331	2.4\\
	1.08	2.41426369881718\\
	1.08357964883805	2.42\\
	1.09603430078143	2.44\\
	1.1	2.44638333471215\\
	1.10859930741898	2.46\\
	1.12	2.47813060305129\\
	1.12119448203973	2.48\\
	1.1339652631489	2.5\\
	1.14	2.50948404536076\\
	1.14679719897211	2.52\\
	1.15967487383745	2.54\\
	1.16	2.54050504736368\\
	1.17274443815689	2.56\\
	1.18	2.57114236240016\\
	1.18585523783962	2.58\\
	1.19903320694555	2.6\\
	1.2	2.6014681039823\\
	1.21238512840317	2.62\\
	1.22	2.63143611891144\\
	1.22578524768915	2.64\\
	1.23925376394326	2.66\\
	1.24	2.66110858798532\\
	1.25289784147309	2.68\\
	1.26	2.6904383774573\\
	1.26659640577296	2.7\\
	1.28	2.71949337036917\\
	1.28035311753867	2.72\\
	1.29429056547336	2.74\\
	1.3	2.74821786345038\\
	1.30829549897098	2.76\\
	1.32	2.77667567018988\\
	1.32236396588701	2.78\\
	1.33656900787151	2.8\\
	1.34	2.80483935114348\\
	1.35088714614085	2.82\\
	1.36	2.83272680617129\\
	1.36527367817563	2.84\\
	1.37973680327023	2.86\\
	1.38	2.86036400830766\\
	1.39437399186818	2.88\\
	1.4	2.88770644451429\\
	1.40908395561573	2.9\\
	1.42	2.91481159798536\\
	1.42386943024178	2.92\\
	1.43875687581496	2.94\\
	1.44	2.94167107690669\\
	1.45379477564742	2.96\\
	1.46	2.96826489209867\\
	1.46891191643103	2.98\\
	1.48	2.99463487788895\\
	1.48411071579356	3\\
	1.49940453082286	3.02\\
	1.5	3.02077893653189\\
	1.51485666763595	3.04\\
	1.52	3.04666877347187\\
	1.53039362135538	3.06\\
	1.54	3.07234725682319\\
	1.54601752941642	3.08\\
	1.56	3.09781777976157\\
	1.56173044065317	3.1\\
	1.57757731953157	3.12\\
	1.58	3.12306108935392\\
	1.5935443299174	3.14\\
	1.6	3.14808863320424\\
	1.60960283744154	3.16\\
	1.62	3.17291958000809\\
	1.62575465266018	3.18\\
	1.64	3.19755702855851\\
	1.6420015103967	3.2\\
	1.65837280268213	3.22\\
	1.66	3.2219893389573\\
	1.6748733644635	3.24\\
	1.68	3.24621772311186\\
	1.6914708952445	3.26\\
	1.7	3.27026299802158\\
	1.70816692544782	3.28\\
	1.72	3.29412800280932\\
	1.72496292024103	3.3\\
	1.74	3.31781552460521\\
	1.74186028189561	3.32\\
	1.75887856405203	3.34\\
	1.76	3.34131856712421\\
	1.77602827378885	3.36\\
	1.78	3.3646348461257\\
	1.79328067386987	3.38\\
	1.8	3.38778299767249\\
	1.81063699604638	3.4\\
	1.82	3.41076558512201\\
	1.82809841737301	3.42\\
	1.84	3.43358512669179\\
	1.84566606207025	3.44\\
	1.86	3.45624409650901\\
	1.86334100330253	3.46\\
	1.88	3.47874492563922\\
	1.8811242648766	3.48\\
	1.89903158957943	3.5\\
	1.9	3.50108201580127\\
	1.91706397366808	3.52\\
	1.92	3.52325764865042\\
	1.93520531209383	3.54\\
	1.94	3.54528331447697\\
	1.95345649395328	3.56\\
	1.96	3.5671612604237\\
	1.97181836491352	3.58\\
	1.98	3.58889369615039\\
	1.99029172857412	3.6\\
	2	3.61048279470147\\
	2.0088773477712	3.62\\
	2.02	3.63193069335429\\
	2.02757594582664	3.64\\
	2.04	3.6532394944479\\
	2.04638820774495	3.66\\
	2.06	3.6744112661926\\
	2.06531478136057	3.68\\
	2.08	3.69544804346048\\
	2.08435627843797	3.7\\
	2.1	3.71635182855715\\
	2.10351327572682	3.72\\
	2.12	3.73712459197497\\
	2.12278631597444	3.74\\
	2.14	3.757768273128\\
	2.14217590889757	3.76\\
	2.16	3.77828478106911\\
	2.16168253211526	3.78\\
	2.18	3.79867599518948\\
	2.18130663204494	3.8\\
	2.2	3.81894376590088\\
	2.20104862476313	3.82\\
	2.22	3.83908991530103\\
	2.22090889683254	3.84\\
	2.24	3.85911623782247\\
	2.2408878060971	3.86\\
	2.26	3.8790245008653\\
	2.26098568244634	3.88\\
	2.28	3.89881644541408\\
	2.28120282855044	3.9\\
	2.3	3.91849378663935\\
	2.30153952056732	3.92\\
	2.32	3.93805821448405\\
	2.32199600882304	3.94\\
	2.34	3.95751139423537\\
	2.34257251846652	3.96\\
	2.36	3.97685496708214\\
	2.36326925009981	3.98\\
	2.38	3.9960905506584\\
	2.38408638038494	4\\
	2.4	4.01521973957327\\
	2.40502406262831	4.02\\
	2.42	4.03424410592764\\
	2.42608242734359	4.04\\
	2.44	4.05316519981799\\
	2.44726158279398	4.06\\
	2.46	4.07198454982755\\
	2.46856161551478	4.08\\
	2.48	4.09070366350541\\
	2.48998259081695	4.1\\
	2.5	4.10932402783355\\
	2.51152455327255	4.12\\
	2.52	4.12784710968251\\
	2.53318752718267	4.14\\
	2.54	4.14627435625565\\
	2.5549715170287	4.16\\
	2.56	4.16460719552256\\
	2.57687650790739	4.18\\
	2.58	4.18284703664184\\
	2.59890246595059	4.2\\
	2.6	4.20099527037348\\
	2.62	4.21904627558988\\
	2.62106165047083	4.22\\
	2.64	4.23700037569099\\
	2.64335575137858	4.24\\
	2.66	4.25486626266903\\
	2.66577171071786	4.26\\
	2.68	4.2726452642721\\
	2.68830940579945	4.28\\
	2.7	4.29033869156097\\
	2.71096869728153	4.3\\
	2.72	4.30794783927118\\
	2.73374942949588	4.32\\
	2.74	4.3254739861665\\
	2.75665143076267	4.34\\
	2.76	4.34291839538383\\
	2.77967451369444	4.36\\
	2.78	4.36028231476996\\
	2.8	4.37754899354514\\
	2.8028498203327	4.38\\
	2.82	4.3947349299427\\
	2.82615040122794	4.4\\
	2.84	4.41184341764745\\
	2.84957237106168	4.42\\
	2.86	4.42887565153436\\
	2.87311546902206	4.44\\
	2.88	4.44583281259827\\
	2.89677942028663	4.46\\
	2.9	4.46271606825016\\
	2.92	4.47952307581562\\
	2.92056999608211	4.48\\
	2.94	4.49623784965642\\
	2.94451650307588	4.5\\
};

==> sections/performance_plot.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
legend columns = 2,
legend style={font=\scriptsize},
width=2.8in,
height=2in,
at={(0.485in,0.481in)},
scale only axis,
xmin=0,
xmax=20,
ymin=-2,
ymax=-1.1,
xlabel={time $t$},
ylabel={cost $L_\pi(x(t),v(t))$},
axis background/.style={fill=white},
legend style={at={(1,0)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, dashed, line width=1.0pt]
  table[row sep=crcr]{%
0	-1.3559665451014\\
1	-1.26299182490599\\
2	-1.22738870581727\\
3	-1.21372173223233\\
4	-1.2084719064055\\
5	-1.20645408421976\\
6	-1.20567757723462\\
7	-1.20537959741291\\
8	-1.20526515131313\\
9	-1.20522037852511\\
10	-1.20520467027561\\
11	-1.20519751427519\\
12	-1.20519508422951\\
13	-1.20519452506239\\
14	-1.20519330652877\\
15	-1.20519412807589\\
16	-1.2051943831783\\
17	-1.20519356566267\\
18	-1.20519310607928\\
19	-1.20519318319181\\
};
\addlegendentry{$L^{\text{max}}_\pi(z,v)), \ell=L_\pi^{\text{max}}$}

\addplot [color=mycolor1, line width=1.0pt]
  table[row sep=crcr]{%
0	-1.35596680110656\\
1	-1.60622521566465\\
2	-1.4675876285722\\
3	-1.59127897111591\\
4	-1.51446840838347\\
5	-1.50820053835822\\
6	-1.32068612083525\\
7	-1.58966137435104\\
8	-1.20898497555151\\
9	-1.33757900217035\\
10	-1.4145428466495\\
11	-1.53322809164975\\
12	-1.31150590053762\\
13	-1.55800972038287\\
14	-1.59152133070381\\
15	-1.29484804499094\\
16	-1.47424378755786\\
17	-1.21055093712757\\
18	-1.39528611343679\\
19	-1.23098691593487\\
};
\addlegendentry{$L_\pi(x,v), \ell=L_\pi^{\text{max}}$}

\addplot [color=mycolor2, dashed, line width=1.0pt]
  table[row sep=crcr]{%
0	-1.39575892177084\\
1	-1.23858785726828\\
2	-1.17704822953637\\
3	-1.1548690028762\\
4	-1.14716764374167\\
5	-1.14453107013311\\
6	-1.14363453889871\\
7	-1.14332508319976\\
8	-1.14322300330114\\
9	-1.14318740611299\\
10	-1.1431737495913\\
11	-1.14316658061052\\
12	-1.14316978720509\\
13	-1.14316882638099\\
14	-1.14316692497803\\
15	-1.14316838042263\\
16	-1.14316906322418\\
17	-1.14316891951597\\
18	-1.14316641589422\\
19	-1.14316722637195\\
};
\addlegendentry{$L_\pi^{\text{max}}(z,v), \ell=L_\pi$}

\addplot [color=mycolor2, line width=1.0pt]
  table[row sep=crcr]{%
0	-1.3957593198278\\
1	-1.66755623631387\\
2	-1.50220234994494\\
3	-1.64669534308848\\
4	-1.55781709569728\\
5	-1.55051483213631\\
6	-1.31237330209738\\
7	-1.64498197911944\\
8	-1.14906346775275\\
9	-1.33557157972321\\
10	-1.43613186492004\\
11	-1.580122466086\\
12	-1.29988186843123\\
13	-1.60886047428345\\
14	-1.64711487055172\\
15	-1.27657175605993\\
16	-1.51000162445669\\
17	-1.15157058158571\\
18	-1.41159137103562\\
19	-1.18307174276809\\
};
\addlegendentry{$L_\pi(x,v), \ell=L_\pi$}

\end{axis}

\begin{axis}[%
width=5.833in,
height=4.375in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%

==> sections/time_plot.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.50000,0.62000,0.22000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=3.123in,
height=2.5in,
at={(0.2in,0.21in)},
legend style={font=\scriptsize},
scale only axis,
xmin=-2,
xmax=19,
ymin=1,
ymax=6,
xlabel={time $t$},
ylabel={state $x$},
axis background/.style={fill=white},
legend style={at={(1.03,0.5)}, anchor=west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=white!85!black,forget plot]
  table[row sep=crcr]{%
-2	2.43142912800101\\
20	2.43142912800101\\
};

\addplot [color=white!85!black, forget plot]
  table[row sep=crcr]{%
-2	4.23442116324993\\
20	4.23442116324993\\
};

\addplot [color=white!85!black,forget plot]
  table[row sep=crcr]{%
-2	3.23442116324993\\
20	3.23442116324993\\
};

\addplot [color=white!85!black, forget plot]
  table[row sep=crcr]{%
-2	2.23442116324993\\
20	2.23442116324993\\
};

\addplot [color=white!85!black,forget plot]
  table[row sep=crcr]{%
-2	1.23442116324993\\
20	1.23442116324993\\
};

\addplot [color=mycolor1, draw=none, mark=square, mark options={solid, mycolor1}, line width=1.0pt]
  table[row sep=crcr]{%
-0.5	3.23442116324993\\
};
\addlegendentry{$\zs\oplus \Omega, \ell =L_\pi^{\text{max}}$}

\addplot [color=mycolor1, line width=1pt, forget plot]
  table[row sep=crcr]{%
-0.5	4.23442116324993\\
-0.5	2.23442116324993\\
};

\addplot [color=mycolor2, draw=none, line width=1, mark=square, mark options={solid, mycolor2}]
table[row sep=crcr]{%
	-1.5	2.23442182886124\\
};

\addlegendentry{$\zs \oplus \Omega, \ell = L_\pi$}

\addplot [color=mycolor2, line width=1pt, forget plot]
table[row sep=crcr]{%
	-1.5	3.23442182886124\\
	-1.5	1.23442182886124\\
};

\addplot [color=mycolor3, draw=none, line width=1, mark=square, mark options={solid, mycolor3}]
table[row sep=crcr]{%
	-1	2.43142912800101\\
};
\addlegendentry{$\zs \oplus \Omega, \ell = L_\pi^{\text{int}}$}

\addplot [color=mycolor3, line width=1pt, forget plot]
table[row sep=crcr]{%
	-1	3.43142912800101\\
	-1	1.43142912800101\\
};

\addplot [color=mycolor1, line width=1.0pt]
table[row sep=crcr]{%
	0	3.23442116324993\\
	1	4.5060291769985\\
	2	4.00630865778998\\
	3	4.73244663466431\\
	4	4.39496155793787\\
	5	4.28040451870974\\
	6	3.2889031240528\\
	7	4.54076690679745\\
	8	2.93262620808584\\
	9	2.98443378171559\\
	10	3.36454728823329\\
	11	4.16924714895533\\
	12	3.22422060184428\\
	13	4.29489317238766\\
	14	4.82712235993904\\
	15	3.31487472249733\\
	16	3.79056792775311\\
	17	2.74795032677564\\
	18	3.19117054060129\\
	19	2.64725950160853\\
};
\addlegendentry{$x(t), \ell=L_\pi^{\text{max}},N=10$, without \eqref{eq:diss_inducing_constr}}

\addplot [color=mycolor1, dotted, line width=1.0pt]
table[row sep=crcr]{%
	0	4.23441989514753\\
	1	5.50602737520545\\
	2	5.00630706654045\\
	3	5.73244473718442\\
	4	5.3949598030241\\
	5	5.280402812094\\
	6	4.28890183323688\\
	7	5.54076509033471\\
	8	3.93262506550549\\
	9	3.98443261762863\\
	10	4.36454596585563\\
	11	5.16924548916309\\
	12	4.22421933799228\\
	13	5.29489145966665\\
	14	5.82712187556483\\
	15	4.31487342085032\\
	16	4.79056642710008\\
	17	3.74794926073654\\
	18	4.19116929051981\\
	19	3.64725945035673\\
};
\addlegendentry{$z(t),\ell=L_\pi^\text{max},N=10$, without \eqref{eq:diss_inducing_constr}}

\addplot [color=mycolor1, densely dashed, line width=1.0pt]
  table[row sep=crcr]{%
0	4.23441989514753\\
1	3.57196850545093\\
2	3.35784109410191\\
3	3.28075527350422\\
4	3.25185859791898\\
5	3.24085523870277\\
6	3.23663927946005\\
7	3.2350235041581\\
8	3.23440240365446\\
9	3.2341631445152\\
10	3.23407330792236\\
11	3.23403668998419\\
12	3.23402417500245\\
13	3.23401954438146\\
14	3.23401699210131\\
15	3.23401851781581\\
16	3.2340171309942\\
17	3.23401425251578\\
18	3.23401410147534\\
19	3.23401527065881\\
};
\addlegendentry{$z(t), \ell=L_\pi^{\text{max}},N=10$}

\addplot [color=mycolor1, dashed, line width=1.0pt]
  table[row sep=crcr]{%
0	4.23442075669701\\
1	3.4810626901621\\
2	3.24364336339431\\
3	3.158863414747\\
4	3.12713427649218\\
5	3.11504379608744\\
6	3.1104047818332\\
7	3.10861907072004\\
8	3.10793388035279\\
9	3.10766885660315\\
10	3.10756560680089\\
11	3.10752438913983\\
12	3.1075098984554\\
13	3.10750444638487\\
14	3.10750124583053\\
15	3.10750139201126\\
16	3.10750273774296\\
17	3.10750243212037\\
18	3.10750266607397\\
19	3.10750224428402\\
};
\addlegendentry{$z(t), \ell=L_\pi^{\text{max}},N=4$}

\addplot [color=mycolor1, loosely dashed, line width=1.0pt]
  table[row sep=crcr]{%
0	4.23442074039515\\
1	3.3260732420691\\
2	3.05254402408926\\
3	2.95626223336334\\
4	2.92032481299355\\
5	2.9066065210152\\
6	2.90132441332838\\
7	2.89928393681695\\
8	2.89849463576053\\
9	2.89818803027543\\
10	2.89807131139329\\
11	2.89802429524104\\
12	2.89801050941687\\
13	2.89800175744841\\
14	2.89799904221289\\
15	2.89799727589194\\
16	2.89799659931697\\
17	2.8979962381419\\
18	2.89799576351308\\
19	2.89799569758819\\
};
\addlegendentry{$z(t), \ell=L_\pi^{\text{max}},N=3$}

\addplot [color=mycolor3, densely dashed, line width=1.0pt]
table[row sep=crcr]{%
	0	3.4314275357731\\
	1	2.72634184467843\\
	2	2.52682629135386\\
	3	2.46322051324879\\
	4	2.44209639162189\\
	5	2.43497681440464\\
	6	2.43256714481514\\
	7	2.43175698058704\\
	8	2.43148003110215\\
	9	2.4313868801699\\
	10	2.43135872017141\\
	11	2.43134247044551\\
	12	2.4313373774971\\
	13	2.43134030357135\\
	14	2.43133844827149\\
	15	2.43133767457929\\
	16	2.43133889018229\\
	17	2.43133817116326\\
	18	2.43134000738379\\
	19	2.43133724098953\\
};
\addlegendentry{$z(t),\ell=L_\pi^\text{int}, N=10$}

\addplot [color=mycolor3, dashed, line width=1.0pt]
table[row sep=crcr]{%
	0	3.43142711809482\\
	1	2.67975392429967\\
	2	2.47021449795244\\
	3	2.403783943929\\
	4	2.38176948470614\\
	5	2.37436354711086\\
	6	2.37185742083677\\
	7	2.37101064635272\\
	8	2.37072301239326\\
	9	2.37062403410202\\
	10	2.37059272423346\\
	11	2.37058124364821\\
	12	2.37057710107185\\
	13	2.37057696885116\\
	14	2.37057460389657\\
	15	2.37057497050181\\
	16	2.37057616671164\\
	17	2.3705755403213\\
	18	2.37057426721103\\
	19	2.37057571719686\\
};
\addlegendentry{$z(t),\ell=L_\pi^\text{int}, N=4$}

\addplot [color=mycolor2, loosely dashed, line width=1.0pt]
  table[row sep=crcr]{%
0	3.23442172572926\\
1	2.40868376709945\\
2	2.17987912591962\\
3	2.10744110883028\\
4	2.0834648863524\\
5	2.07540864527325\\
6	2.07268814844399\\
7	2.07176992117404\\
8	2.07145670308366\\
9	2.07135029466235\\
10	2.07131544369468\\
11	2.07130180218883\\
12	2.07130106071775\\
13	2.07130126232757\\
14	2.07129784230085\\
15	2.07129672868655\\
16	2.07130069917971\\
17	2.07129717071485\\
18	2.07129705422949\\
19	2.07129667789424\\
};
\addlegendentry{$z(t),\ell = L_\pi, N=3$}

\addplot [color=mycolor2, dashed, line width=1.0pt]
  table[row sep=crcr]{%
0	3.23441980269994\\
1	2.49227931711642\\
2	2.28100548295656\\
3	2.2133595224511\\
4	2.19083052371068\\
5	2.183225615823\\
6	2.18064605737843\\
7	2.17977266518964\\
8	2.17947416485267\\
9	2.17937347604946\\
10	2.17933914063302\\
11	2.17932870593098\\
12	2.17932231760942\\
13	2.17932291786775\\
14	2.17932158534149\\
15	2.17931964095393\\
16	2.17932195846766\\
17	2.1793217102586\\
18	2.17932186993934\\
19	2.17932309700982\\
};
\addlegendentry{$z(t),\ell = L_\pi, N=4$}

\addplot [color=mycolor2, densely dashed, line width=1.0pt]
  table[row sep=crcr]{%
0	3.23442022149185\\
1	2.53378674725079\\
2	2.33195510692551\\
3	2.26705491857592\\
4	2.24540748110971\\
5	2.23809729325646\\
6	2.23561798446614\\
7	2.23476876674951\\
8	2.23448365171561\\
9	2.234383238714\\
10	2.23434635104473\\
11	2.23433378208978\\
12	2.23433850661383\\
13	2.23433543825845\\
14	2.23433307925146\\
15	2.23433638661984\\
16	2.2343367134537\\
17	2.23433394580788\\
18	2.23433141226104\\
19	2.23433468461869\\
};
\addlegendentry{$z(t),\ell = L_\pi, N=10$}

\addplot [color=mycolor2, line width=1.0pt]
  table[row sep=crcr]{%
0	2.23442182886124\\
1	3.46784768480447\\
2	2.42641989499205\\
3	3.21242476546233\\
4	2.67504058435281\\
5	2.63355605471299\\
6	1.66779725337344\\
7	3.18731878725967\\
8	1.24694555030545\\
9	1.74034824107422\\
10	2.10392969344231\\
11	2.793100736083\\
12	1.62970893340191\\
13	2.96032218704414\\
14	3.20113554450424\\
15	1.56202114701633\\
16	2.42900487991482\\
17	1.25230752918321\\
18	2.00747425528437\\
19	1.32265591065714\\
};
\addlegendentry{$x(t),\ell = L_\pi, N=10$}

\end{axis}
\end{tikzpicture}%
